CANdito: Improving Payload-based Detection of Attacks on Controller Area Networks

Over the years, the increasingly complex and interconnected vehicles raised the need for effective and efficient Intrusion Detection Systems against on-board networks. In light of the stringent domain requirements and the heterogeneity of information transmitted on Controller Area Network, multiple approaches have been proposed, which work at different abstraction levels and granularities. Among these, RNN-based solutions received the attention of the research community for their performances and promising results. In this paper, we improve CANnolo, an RNN-based state-of-the-art IDS for CAN, by proposing CANdito, an unsupervised IDS that exploits Long Short-Term Memory autoencoders to detect anomalies through a signal reconstruction process. We evaluate CANdito by measuring its effectiveness against a comprehensive set of synthetic attacks injected in a real-world CAN dataset. We demonstrate the improvement of CANdito with respect to CANnolo on a real-world dataset injected with a comprehensive set of attacks, both in terms of detection and temporal performances.

==> Sections/cannolo.tex <==
\section{Cannolo + [Motivation]}
\sk{descrizione brief + cannolo analysis and limitations [1 pagina]}

% In  this  section,  we  provide  an  overview  of  CANnolo, highlighting the core concepts necessary for the understanding of CANdito. We refer the interested reader to [4] for a more in depth analysis


% \begin{figure}
% 	\centering
% 	\includegraphics[width=\linewidth]{Images/Approach.pdf}
% 	\caption{Overview of \oldsystem's detection process, from~\cite{longari2020cannolo}.}
% 	\label{fig:autoencoderoverview}
% \end{figure}

% Figure~\ref{fig:autoencoderoverview} shows an overview of the architecture of \oldsystem, which works by reconstructing time series of CAN packets for each ID and computes their anomaly score based on the reconstruction error. 
% It is composed of two main modules: an LSTM-based autoencoder, which learn the legitimate signal behaviour, and a anomaly detector, which compares the reconstruction errors.  

% \mypar{LSTM-based autoencoder}
% Based on the works of Malhotra et al.~\cite{malhotra2016lstm}, \oldsystem is composed of an autoencoder architecture, with two recurrent LSTM layers for both the encoder and the decoder.  
% Due to the temporal nature of \ac{CAN} data, the input is fed to the system through a rolling window of 40 CAN packets. Each packet consists in at most $k=64$ bits, depending on the CAN ID under analysis.  
% The encoder is  composed of a dense layer, consisting of $C=256$ units with hyperbolic tangent activation  functions, followed by a $20\%$ dropout layer and two recurrent LSTM layers with $L=128$ units each. Symmetrically, the decoder consists of two recurrent LSTM layers with $L=128$ units each and a dense layer, consisting of $C=256$ units with sigmoid activation functions (to scale the results to the [0,1] interval). 

% \begin{figure}
% 	\centering
% 	\includegraphics[width=0.7\linewidth]{Images/CANnoloLSTM}
% 	\caption{Autoencoder architecture.}
% 	\label{fig:architecture}
% \end{figure}


% The reconstruction error distribution is calculated using only legitimate data from the validation set. 

% The resulting mean $\mu$ and covariance $\Sigma$ matrixes indicate the multivariate Gaussian distribution of the non-anomalous data. 

% A Mahalanobis distance between this distribution and any given reconstruction error distribution from a test sequence will suffice to identify  an anomaly. 

\subsection{Anomaly detector}

The anomaly detector works by computing the statistical characteristics of reconstruction errors over a separate validation dataset; then, it assigns a distance score that indicates how far a given reconstruction error is from the expected normal distribution. 
autoencoders do not use any validation data  with anomalous traffic to tune the anomaly signal. Instead, the inhere proposed \oldsystem is a completely unsupervised approach to anomaly detection.


\subsection{Anomaly signal processing}
\label{autoencoder-signal}

The anomaly detection procedure consists in calculating the Mahalanobis distance 
between two sequences. For a single reconstruction, unlike Malhotra's approach~
\cite{malhotra2016lstm}, a binary cross-entropy function is employed. Early tests 
suggested that this function is to be preferred to the absolute error function used 
by the authors \cite{malhotra2016lstm}. Formally:
$$-(\hat{b}_k\log(b_k+\epsilon)+(1-\hat{b}_k)\log(1-b_k)+\epsilon)$$
where $\hat{b}_k$ is the k-th bit in the reconstructed sequence $\hat{y}^{(t)}$ and $b_k$ is the k-th bit of the source sequence $s^{(t)}$.

\mypar{Normal reconstruction error distribution}
A dataset consisting only of legitimate data sequences has been used as the baseline to  
establish the `normal' behaviour for any given CAN ID. The reconstruction error 
distribution has been extracted from the join list of reconstruction errors as 
described above. The distribution is thus fitted to a multivariate Gaussian 
distribution, providing the mean $\mu$ (of $1\times k$ cardinality) and covariance 
matrix $\Sigma$ (of $k \times t$ cardinality).

% TODO @skizzo: modifica creando una sola figura \label{fig:anomdistributions} composta da una colonna di 3 sugfibures {fig:anomdistributions:normal}, {fig:anomdistributions:interleave}, {fig:anomdistributions:replay}.

\mypar{Anomaly score}
The anomaly score indicates the likelihood of the test sequence to be anomalous. 
Similarly to \cite{malhotra2015long,malhotra2016lstm}, an anomaly score $a$ is derived 
from the Mahalanobis distance measuring the distance between a reconstruction error and 
the distribution of normal/legitimate errors, and it is computed as follows:

$$ a = (e-\mu)^T \Sigma^{-1}(e-\mu)$$
Where $e$ is the reshaped reconstruction error vector.

\begin{figure}
\caption{Anomaly score distribution for various test sequences.}
\label{fig:overallanomaly}
	\begin{subfigure}[b]{0.5\textwidth}
		\centering
		\includegraphics[width=0.65\linewidth]{Images/normal}
		\caption{Anomaly score distribution for test sequences with normal data.}
		\label{fig:normal}
	\end{subfigure}

	\begin{subfigure}[b]{0.5\textwidth}
		\centering
		\includegraphics[width=0.65\linewidth]{Images/interleave}
		\caption{Anomaly score distribution for test sequences with an interleave anomaly.}
		\label{fig:interleave}
	\end{subfigure}
	\begin{subfigure}[b]{0.5\textwidth}
		\centering
		\includegraphics[width=0.65\linewidth]{Images/replay}
		\caption{Anomaly score distribution for test sequences with a replay attack targeting a high variability field.}
		\label{fig:replay}
	\end{subfigure}

\end{figure}


Figure \ref{fig:overallanomaly} presents three sample distributions. 

Firstly, in Figure \ref{fig:normal}, the baseline reconstruction error is presented showing that the distance between the source and the reconstructed sequences are generally low. 

Secondly, in Figure \ref{fig:interleave}, an interleave anomaly is presented. % TODO @skizzo: giustificazione errore?

Finally, Figure \ref{fig:replay} presents a replay anomaly. By comparison with Figure \ref{fig:normal}, it is clear that the sequences are recognized as legitimate but temporally misplaced (low reconstruction errors interleaved with high reconstruction errors on anomaly's boundaries). 

\subsection{Cannolo's analysis}
solo testo

==> Sections/implementation.tex <==

\section{RNN autoencoder-based IDS} \label{rnnimplementation}
The module has been implemented using the Python \ac{ML} library Tensorflow-gpu (version 2.1)~\cite{tensorflow} with its module for the \ac{NN} \acs{API} Keras.
\par
As we said in Section~\ref{rnnapproach} this module is based on CANnolo by Longari et al.~\cite{longari2020cannolo}, because their model was proven to provide interesting results on the same problem. Starting from this model we developed four new versions, each one of them either improving the detection capabilities or reducing the detection time of the network. For the sake of our thesis, we just present our final version of the model and the differences from the original model, explaining the reasons behind these changes; however, it is important to underline that all these changes were not implemented in a single iteration, but were part of a process that led us to improve the network in different steps, each one evaluated by itself to improve the previous one is some aspects. 
\par
Our code has been thought in a way that the different versions of the model use the same basic functions for training, threshold computation, and detection, with only specific parts that are modified to behave differently for different versions of the model. In particular, the main differences between the original model (CANnolo) and our system are:
\begin{itemize}
    \item The number of the artificial neurons of all layers has been halved (see Figures~\ref{fig:autoencoderids} and Figure~\ref{fig:cannoloids}). The reduction of the dimension of the layers has a twofold scope: as we noticed that the networks of several \acp{CAN-ID} were prone to overfitting, reducing the dimension of the layers mitigated this problem; moreover, reducing the dimension of the layers has a substantial impact on the improvement of the training and testing times of the network.
    \item The activation functions of the two symmetric dense layers of the encoder and decoder have been modified from hyperbolic tangent to \ac{ELU}; this choice has been made because this function has been proven to mitigate the vanishing gradient problem and to improve the generalization capabilities of the network~\cite{clevert2015fast},~\cite{hanselmann2020canet}.
    \item The inputs of the original network are bit-strings composed of the condensed notation (i.e., without constant bits) of the packets. In our solution not only the constant bits (that do not belong to any signal) are excluded, but also the signals marked by READ as counters or \acp{CRC}; the idea behind this decision is that counters and \acp{CRC} do not carry interesting information for the \ac{NN}, as considering them did not improve the effectiveness of the system. The input is not composed by bit-strings, but by each signal of the \ac{CAN-ID} rescaled in the 0-1 range. This allows to reduce the dimension of the input by a lot (e.g., for some \acp{CAN-ID} the input was in the order of 40 bits for the original network that become only 4 signals with the modified input), reducing significantly the testing and training times of the network. The tests performed with the input modified this way have not shown meaningful effects on the detection performance.
    \item The output sequence of the encoder is reversed before being fed into the decoder; this operation is meant to help the network reconstructing the target sequence, which is also reversed as suggested by Sutskever et al.~\cite{sutskever2014sequence}. While the results of the networks of some \ac{CAN-ID} were about the same with or without this reversion of the encoder output, some other networks went from having serious underfitting problems to performing good generalization after this change. 
    \item differently from CANnolo we do not feed the reconstructed sequence back into the decoder in order to further reduce the dimension of the inputs and the computational effort needed.
\end{itemize}
\par
An important detail of our implementation is that in order to improve the variety of the data the training sequences are taken from different takes of real \ac{CAN} traffic, in particular the datasets number 1, 2, 6, 8, and 9 of the ReCAN C-1 dataset~\cite{zago2020recan}, that amount approximately 105 minutes of \ac{CAN} traffic. 
\par
The first step to build the input sequences is applying the READ algorithm (presented in Section~\ref{read}) to associate to each \ac{CAN-ID} the corresponding ranges of the signals. Using this information the payloads of each packet are converted into the list of their signals, excluded counters and \acp{CRC}, rescaled in the 0-1 range. Then, for each of the datasets separately, the input training sequences are created sliding by one step at a time a window of dimension \(\mathit{n=40}\) packets over the dataset, in a way that each packet is contained in \textit{n} input sequences of dimension \textit{n} x \textit{k}. The training windows created this way are concatenated, then they are shuffled before each epoch of the training process. The windows for the testing data are computed in the same way, with the difference that the windows do not overlap.

==> Sections/threat.tex <==
\section{Threat Model}
\label{sec:threat}

As said in Chapter~\ref{chapter:intro} modern vehicles have both a wide internal and external attack surface and, while in most cases adversaries have not direct access to the internal network (except in particular cases as car-sharing services), more and more options are available as the cars become more connected. While securing all the different components of the attack surface is fundamental, it must be considered that all those technologies are heterogeneous and diverse; we will instead concentrate on what happens on the \ac{CAN} bus, assuming that one or more \acp{ECU} have been compromised, no matter the channel through the attack has been effectively performed.
\par
This considered our scope will be to evaluate the effectiveness of different kinds of \acp{IDS} that analyze the packet traffic on in-vehicle networks and, in particular, the \ac{CAN} bus, as it is the predominant technology in the industry. To do so, we will not only consider the possible threats, but we will also concentrate on the possible answers to them.
\par
In order to better define our focus, while attacks on the \ac{CAN} bus can be both performed through normal and diagnostic messages~\cite{miller2016can}, we will consider only the former. Miller and Valasek~\cite{miller2016can} suggested that a possible solution to attacks performed through diagnostic messages may be having a ''diagnostic mode'' to allow them only when their use is needed. This considered focusing only on normal messages does not seem an excessive assumption. Finally, while different \acp{ECU} may be located on different buses (e.g., Low speed and High-speed \ac{CAN}) it has been demonstrated that an attacker can gain access to the more sensitive High-speed \ac{CAN} through an \ac{ECU} that is on both networks (e.g., Telematics)~\cite{koscher2010experimental}, for this reason we will not distinguish between the different sub-networks.
\par
We will consider an adversary model where the attacker has already compromised at least one \ac{ECU} and can be of two different types:
\begin{itemize}
    \item \textit{Weak adversary}: a weak attacker has access to the \ac{CAN} bus directly or through a compromised \ac{ECU}, but his target \ac{ECU} is not compromised in a way that makes it incapable of sending messages on the bus. This means that a weak attacker, whatever his knowledge of the protocol and of the semantics of the messages, will need to change the frequency of the messages of the target \ac{CAN-ID} on the bus in order to succeed in his exploitation.
    \item \textit{Strong adversary}: a strong attacker has also access to a weakly compromised \ac{ECU} and she can prevent it from sending messages. This means that she has all the capabilities of a weak attacker, while also being able to suppress the messages from the target \ac{ECU} and spoofing it without changing the frequency of messages on the bus.
\end{itemize}
\par
As we discussed in Section~\ref{sec}, by design the \ac{CAN} protocol lacks some basic security properties. This means that every adversary with access to the network has some basic capabilities:
\begin{itemize}
    \item \textit{Sniffing}: as \ac{CAN} is a broadcast protocol that lacks any cryptography mechanism, anyone that has access to the bus is able to listen to the messages sent by any \ac{ECU}.
    \item \textit{Packet Injection}: as \ac{CAN} protocol lacks any form of authentication, any node can send messages on the bus with any \ac{CAN-ID}, being potentially able to impersonate any other \ac{ECU} on the network.
\end{itemize}
\par
Addressing those issues is problematic because it would need drastic and expensive modifications of the protocol. This means that on most vehicles even a weak adversary has access to a wide range of different attacks: 
\begin{itemize}
    \item \textit{Spoofing Attack}: in order to try to impersonate a target \ac{ECU}, the attacker floods the network with messages with the same \ac{CAN-ID} as the target. If the injection rate is higher enough than the normal frequency of the target messages the other \acp{ECU} will read the injected messages.
    \item \textit{Fuzzing Attack}: this attack consists of injecting random or partially random messages on the network, in order to cause malfunctions. This method has also been used to try to reverse engineer the semantics of the messages~\cite{koscher2010experimental}.  
    \item \textit{\acf{DoS}}: similar to the previous attacks, but as the objective is to saturate the network the injection rate is higher and the \ac{CAN-ID} of the injected messages is low (even 0) as the arbitration mechanism of the \ac{CAN} protocol gives priority to messages with lower \ac{CAN-ID}.
    \item \textit{Drop attack}: the compromised ECU is prevented from sending messages (e.g,. by putting it into Bootrom mode~\cite{miller2016can} or with a targeted \ac{DoS} attack~\cite{palanca2017stealth}).
\end{itemize}
As the first step for these types of attack to be successful they must conform to the protocol and to various rules that would make \acp{ECU} refuse the new packets. Several rules can be checked by an \ac{IDS} in order to easily refuse those malformed messages, for example by checking their formal correctness with regard to \ac{CAN} specification (correct size of sections, field delimiters, bit stuffing, \ac{CRC}), the consistency of eventual counters and \ac{CRC} in the payload (while often if there are problems in these sections the \ac{ECU} will just reject the messages) and of bits that are never used. Even for messages that are formally correct, these types of attack are easily and reliably detected by simple classifiers taking into account the increased (for spoofing, fuzzing, and \ac{DoS}) or decreased (for drop) frequency of messages of the target \ac{CAN-ID} on the bus. This means that for those types of attacks using complex machine algorithms is redundant, as they can be detected with much more simple and fast methods.
\par
As said strong adversaries, besides all the described attacks, have also the possibility of performing more sophisticated \textit{masquerade attacks} (i.e., an impersonation of an \ac{ECU} preserving the frequency of messages). As differently from attacks that widely impact the traffic on the network this type of intrusion is very difficult to be detected by basic intrusion detection approach, an adversary of this type may try to shape the payload of the sent messages in such a way that makes it difficult also for more complex systems to detect the attack. Some of those are:
\begin{itemize}
    \item \textit{Replay Attack}: the payload of the sent messages is replaced with a time series of messages of the same \ac{CAN-ID} previously sniffed on the bus. This type of attacks is intended to trick the \ac{IDS} into considering the injected traffic as valid.
    \item \textit{Continuous Change Attack}: a signal inside the payload of the messages is slowly modified until the wanted malicious value is reached. This type of attack is much more complex as the attacker needs to know the position of a signal inside the payload and its semantics. An attack of this type may make an \ac{IDS} believe that the traffic is valid as no abrupt changes in the value of the signal can be detected.
\end{itemize}
